OWL (Observe, Watch, Listen): Audiovisual Temporal Context for Localizing Actions in Egocentric Videos

Egocentric videos capture sequences of human activities from a first-person perspective and can provide rich multimodal signals. However, most current localization methods use third-person videos and only incorporate visual information. In this work, we take a deep look into the effectiveness of audiovisual context in detecting actions in egocentric videos and introduce a simple-yet-effective approach via Observing, Watching, and Listening (OWL). OWL leverages audiovisual information and context for egocentric temporal action localization (TAL). We validate our approach in two large-scale datasets, EPIC-Kitchens, and HOMAGE. Extensive experiments demonstrate the relevance of the audiovisual temporal context. Namely, we boost the localization performance (mAP) over visual-only models by +2.23% and +3.35% in the above datasets.

==> figures/block.tex <==
\begin{figure}[t!]
 \captionsetup[subfloat]{font=scriptsize,labelfont=scriptsize}
\begin{center}
\includegraphics[width=0.45\textwidth, clip]{images/block.pdf}
\end{center}
\small
% \vspace{-3mm}
\caption{\textbf{Separate-stage framework for temporal action localization.} Proposal generation:  given a sequence of snippet features, action proposals with start/end timestamps are produced. Proposal classifier: given a set of proposal features, classification scores for each proposal are produced. }
% \vspace{-5mm}
\label{figure:block}
\end{figure}
% \chen{Replace `input' using video snippets; annotate that the circles are proposals.} \chen{We need an arrow from input to proposal classifier}

==> figures/context.tex <==
\begin{figure}[t!]
\begin{center}
\includegraphics[width=0.6\textwidth, clip]{images/context.pdf}
\end{center}
\small
\caption{\textbf{The proposed transformer-based proposal classifier.} We input the auditory sequence (yellow) into the encoder and the visual sequence (blue) into the decoder. $K, V$, and $Q$ refer to the components of multi-head attention as in \cite{vaswani2017attention}. The transformer encoder and decoder first perform a self-attention mechanism to enrich the intra-modal representations. Then, the decoder performs multi-head cross-attention to exchange these representations. The amount of context within which self-attention and cross-attention are being performed can be controlled by the attention mask of size $M \times M$, where $M$ is the input sequences size.}
\label{figure:context}
\end{figure}

==> supplementary_sections/homage_context.tex <==
\section{Ablation of temporal context in HOMAGE}
\label{sec:homage_abl}
Similarly to Sec.~\textcolor{red}{4.3} (\cf the main manuscript), we study the effect of the temporal context on the validation set of HOMAGE. In Tab.~\ref{tab:homage_context_size} we ablate the attention window size
$W$. Similarly to our results on EPIC-KITCHEN, increasing $W$ improved the performance and reached its peak of $9.59$ with $W = 4$. Increasing $W$ further slowly diminishes the performance. 


==> supplementary_sections/implementation.tex <==
\section{Implementation details of HOMAGE experiments}
\label{sec:homage_impl}

First, we want to note that action annotations for HOMAGE are not decomposed into nouns and verbs as in EK100. Therefore, we adapt our model to directly provide  predictions for each action class. We train our model for 446 (out of 453) classes, as we removed some videos from the dataset due to the issues with their metadata.  
Similarly to EK100, we extract SlowFast visual \cite{feichtenhofer2019slowfast} and SlowFast auditory features \cite{kazakos2021slow} for the experiments on HOMAGE. The auditory features are extracted with  backbone pre-trained on VGG-Sound \cite{chen2020vggsound}, and the visual features with pre-trained backbones on EK100 \cite{damen2021rescaling}. We use features extracted at 1 FPS for both proposal generation and classification. For the proposal generator, we use a sliding window of size 160 and a stride of 80. 

==> supplementary_tables/homage_context_window_size.tex <==
\begin{table}[h!]
\tabcolsep=0.1cm
\centering
\caption{\textbf{The effect of attention window size W} in the transformer block described in Sec.~\textcolor{red}{3.3}. We report the performance on the validation set, measured by the average mAP ($\%$). Each token on the attention pattern can attend to $\frac{W}{2}$ tokens from each side. }
\small
\begin{tabular}{r|c|c|c|c|c|c|c|c}
     \toprule
     W      &  0   &   2  &     4         &   5   &   6    &      7   &     8    &    9  \\
     \toprule
     Action mAP & 8.17 & 9.11 & \textbf{9.59} & 9.43  &  9.46  &    9.07  &   8.78   &   8.64 \\
    \bottomrule
\end{tabular}
\label{tab:homage_context_size}
\end{table}

==> tables/context.tex <==
\begin{table}[t]
\centering
\caption{\textbf{The effect of attention window.} (temporal context) size W on in the transformer block described in Sec.~\ref{subsec:context}. We report the performance on the validation set, measured by the average mAP ($\%$). Each token on the attention pattern can attend to $\frac{W}{2}$ tokens from each side. }
\small
\begin{tabular}{r|ccc}
 \toprule
 W & Noun & Verb & Action  \\
  \midrule
0 & 12.52 & 11.86 & 8.21 \\
2 & 12.90 & 10.85 &	8.51 \\
4 & 13.33 & 11.60 & 8.71 \\
8 & 13.45 & 11.74 & 8.84 \\
16 & 13.32 & 11.39 & 8.90 \\
32 & 13.22 & 12.15 & 9.06 \\
64 & \textbf{13.96} & 11.67 & \textbf{9.29}\\
128 & 13.89 & \textbf{12.16 } & 8.78 \\
256 & 13.23 & 11.64 & 8.58 \\
512 & 12.64 & 11.53 & 8.66 \\
% \midrule
\bottomrule
\end{tabular}


\label{tab:context_size}
\end{table}

==> tables/supp_ab.tex <==
\begin{table*}[!ht]

\caption{\textbf{Action localization results.}  measured by mAP@tIoU ($\%$) for tIoU $\in{(0.1, 0.2, 0.3, 0.4, 0.5)}$ and the average mAP on the validation and test sets.  For reporting results on the test set, we \textbf{do not use} validation set for training, compared to~\cite{damen2021rescaling}. Second column indicates feature backbones used for the ablation: TSN~\cite{TSN2016ECCV}, I3D~\cite{carreira2017quo}, SF(A)~\cite{kazakos2021slow}, SF(V)~\cite{feichtenhofer2019slowfast}.}

\begin{subtable}{\linewidth}
\centering
\small
\tabcolsep=0.19cm

% \renewcommand{\arraystretch}{0.4}
% \setlength{\tabcolsep}{0.5em}
    \begin{tabu}{r|c|cccccc|cccccc}
        \toprule
Method & Features & \multicolumn{6}{c}{mAP (Val) for Noun classes} &
         \multicolumn{6}{c}{mAP (Test) for Noun classes}  \\
&  & @0.1  &  @0.2  &  @0.3 &  @0.4 &  @0.5  & Avrg. &
    @0.1  &  @0.2  &  @0.3 &  @0.4 &  @0.5  & Avrg. \\
\midrule
Damen \etal~\cite{damen2021rescaling} &  TSN,SF(V) &
        10.31 & 8.33 & 6.17 & 4.47 & 3.35 & 6.53 &
        11.99 & 8.49 & 06.04 & 4.10 & 2.80 & 6.68 \\
AGT~\cite{nawhal2021activity} & I3D &
        11.63 & 9.33 & 7.05 & 6.57 & 3.89 & 7.70 & 
        - & - & - & - & - & - \\
Ours &  SF(A,V) &
        \textbf{17.94 }& \textbf{15.81} & \textbf{14.14} & \textbf{12.13} & \textbf{9.80} & \textbf{13.96} &
        \textbf{16.78} & \textbf{15.22} & \textbf{13.60} &\textbf{ 11.64} & \textbf{9.74} & \textbf{13.40} \\
\bottomrule
\end{tabu}
\caption{Noun}

%  \centering
\end{subtable}
 
\begin{subtable}{\linewidth}
\centering
\small
\tabcolsep=0.2cm

% \renewcommand{\arraystretch}{0.4}
% \setlength{\tabcolsep}{0.5em}
    \begin{tabu}{r|c|cccccc|cccccc}
        \toprule
Method & Features &\multicolumn{6}{c}{mAP (Val) for Verb classes} &
         \multicolumn{6}{c}{mAP (Test) for Verb classes}  \\
&  & 0.1  &  0.2  &  0.3 &  0.4 &  0.5  & Avrg. &
  0.1  &  0.2  &  0.3 &  0.4 &  0.5  & Avrg. \\
\midrule
Damen \etal~\cite{damen2021rescaling} &  TSN + SF&
        10.83 & 9.84 & 8.43 & 7.11 & 5.58 & 8.36 &
        11.10 & 9.40 & 7.44 & 5.69 & 4.09 & 7.54  \\

AGT~\cite{nawhal2021activity} & I3D &
        12.01 & 10.25 & 8.15 & 7.12 & 6.14 & 8.73  & 
        - & - & - & - & - & - \\
Ours & SF(A,V) &
        \textbf{14.48} & \textbf{13.05} & \textbf{11.82} & \textbf{10.25} & \textbf{8.73} & \textbf{11.67} &
        \textbf{16.78 }& \textbf{15.43} & \textbf{14.01} & \textbf{12.73} & \textbf{11.24} & \textbf{14.04} \\
\bottomrule
\end{tabu}
\caption{Verb}
 \end{subtable}
 
\begin{subtable}{\linewidth}
      \centering
      \small
      \tabcolsep=0.23cm

    \begin{tabu}{r|c|cccccc|cccccc}
        \toprule
Method & Features & \multicolumn{6}{c}{mAP (Val) for Action classes} &
         \multicolumn{6}{c}{mAP (Test) for Action classes}  \\
 & & 0.1  &  0.2  &  0.3 &  0.4 &  0.5  & Avrg. &
  0.1  &  0.2  &  0.3 &  0.4 &  0.5  & Avrg. \\
\midrule
Damen \etal~\cite{damen2021rescaling} &  TSN,SF(V) &
        6.95 & 6.10 & 5.22 & 4.36 & 3.43 & 5.21 &
        6.40 & 5.37 & 4.41 & 3.36 & 2.47 & 4.40 \\

AGT~\cite{nawhal2021activity} & I3D &
        7.78 & 6.92 & 5.53 & 4.22 & 3.86 & 5.66 &
        - & - & - & - & - & - \\
Ours & SF(A,V) &
        \textbf{11.01} & \textbf{10.37} & \textbf{9.47} & \textbf{8.24} & \textbf{7.26} & \textbf{9.29} &
      \textbf{ 9.69} & \textbf{9.03} & \textbf{8.07} & \textbf{7.11} & \textbf{6.23} & \textbf{8.03} \\

\bottomrule
\end{tabu}
 \caption{Action}
 \end{subtable}
\label{tab:sota}
\end{table*}




